Speed-up of Data Analysis with Kernel Trick in Encrypted Domain

Homomorphic encryption (HE) is pivotal for secure computation on encrypted data, crucial in privacy-preserving data analysis. However, efficiently processing high-dimensional data in HE, especially for machine learning and statistical (ML/STAT) algorithms, poses a challenge. In this paper, we present an effective acceleration method using the kernel method for HE schemes, enhancing time performance in ML/STAT algorithms within encrypted domains. This technique, independent of underlying HE mechanisms and complementing existing optimizations, notably reduces costly HE multiplications, offering near constant time complexity relative to data dimension. Aimed at accessibility, this method is tailored for data scientists and developers with limited cryptography background, facilitating advanced data analysis in secure environments.

==> Sections/04_our_model.tex <==
\section{\texorpdfstring{$\phi$-ZER}{Phi-ZER}}
% \section{$\phi$-ZER}

\subsection{Overview}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/phizer_framework.eps}
    \caption{Our framework, $\phi$-ZER, calculates the time complexities of an algorithm's general and kernel evaluation in a homomorphic encryption scheme, and selects the evaluation method that yields the best time performance.}
    \label{fig:phizer_framework}
\end{figure}

Our framework, $\phi-$ZER, is a secure two-party computation over the homomorphic encryption scheme. We assume a semi-honest security model, which is a general threat model setting as described in~\cite{aono2017privacy}. 

\subsubsection{Client}
% \textcircled{\small{1}} \textbf{Client.} 
We assume that the client has a dataset $\textbf{D} = \{ \mathbf{x}_i \}_{i=1}^{n}$ and a set of queries $Q$. The client performs a tuple of algorithms: (\textsf{KeyGen}, \textsf{Encrypt}, \textsf{Decrypt}). 

\begin{itemize}[leftmargin=0.4cm]
    \item $\textsf{KeyGen}(\lambda) \rightarrow (sk, pk, evk)$. The client generates a tuple of a secret key $sk$, a public key $pk$, and an evaluation key $evk$ based on the security level $\lambda$.
    \item $\textsf{Encrypt}(\textbf{D}, pk) \rightarrow \textbf{C}$. The client uses the public key $pk$ to encrypt each data $\mathbf{x}_i \in \textbf{D}$ and obtain ciphertext $\mathbf{c}_i \in \textbf{C}$.
    \item $\textsf{Decrypt}(\mathbf{c}^*, sk) \rightarrow {q(\textbf{D})}$. The client receives ciphertext $\mathbf{c}^*$ such that the decryption outputs the result of their query $q \in Q$.
\end{itemize}
%
The client sends the encrypted data \textbf{C}, the public key $pk$, the evaluation key $evk$, and a set of queries $Q$ to the server.

\subsubsection{Server}
% \textcircled{\small{2}} \textbf{Server.} 
$\phi$-ZER, consists of two stages: \emph{kernel selection} and \emph{evaluation} (see Fig.~\ref{fig:phizer_framework}). The selection phase involves deciding on pathfinding for the circuit evaluation, either using the general circuit or the kernel circuit. The selection process precedes the evaluation phase, during which the selected circuit is used for time-efficient computation based on the optimization result.

\noindent \textbf{Kernel Selection Step}. The server conducts a \emph{Kernelization} process that consists of calculating time complexities.

$\underline{\textsf{Kernelization}(\textbf{C}, Q, evk) \rightarrow \mathbb{B}}$
%
\begin{itemize}[leftmargin=0.35cm]
    \item \textsf{KZ.GeneralPerf($Q$)} $\rightarrow t_{gen}$. The algorithm computes time complexity $t_{gen}$ of the general evaluation of user queries $Q$. 
    \item \textsf{KZ.KernelPerf($Q$)} $\rightarrow t_{ker}$. The algorithm computes time complexity $t_{ker}$ of the kernel evaluation of user queries. 
    \item \textsf{KZ.KernelDecision}($t_{gen}, t_{ker}$) $\rightarrow \mathbb{B}$. The server compares time complexities $t_{gen}, t_{ker}$, and outputs $\mathbb{B} = \{0, 1\}$ corresponding to the queries $Q$ where general and kernel circuit evaluation refers to $0$ and $1$, respectively.
\end{itemize}

\noindent \textbf{Evaluation Step}. The server evaluates the client's query $q \in Q$ based on the parameter $\mathbb{B}$ obtained from the kernel selection step. If the parameter $\mathbb{B}$ promotes the kernel circuit evaluation, $\phi$-ZER performs the following sub-module. 

$\underline{\textsf{KernelEval}(1 \in \mathbb{B}, \textbf{C}, Q, evk) \rightarrow \mathbf{c}^*}$
%
\begin{itemize}[leftmargin=0.35cm]
    \item $\textsf{KE.ParallelKer}(\mathbf{C}, n) \rightarrow \mathbf{K}$. Assuming that the server has sufficient computation power, the following holds:
    \begin{itemize}[leftmargin=0.1cm]
        \item Allocate all ciphertext pair $(\mathbf{c}_i, \mathbf{c}_j)$ to each processor $proc_{k}$.
        \item For each $\{ proc_{k} \}_{k=1 \dots \frac{n(n+1)}{2}}$, evaluate encryption of $K(\textbf{x}_i, \textbf{x}_j)$ using their corresponding ciphertext $\textbf{c}_i$ and $\textbf{c}_j$. 
    \end{itemize}
    \item $\textsf{KE.EvalAlg}(\mathbf{K}, Q, evk) \rightarrow \mathbf{c}^*$. The server performs kernel\! evaluation\! with the evaluation key $evk$ and outputs $\mathbf{c}^*$.
\end{itemize}



% \noindent\textbf{Memory Efficient.} Once our optimizer decides to perform either general or kernel method, holding both the dataset $\textbf{D}$ and the kernel matrix $\mathbf{K}$ is unnecessary. Thanks to the symmetric property of the kernel matrix, when $d > \frac{n+1}{2}$, it consumes less memory to store the kernel matrix than the data matrix.


==> Sections/08_discussion.tex <==
\section{Discussion}
\label{section:discussion}
 % \subsection{$\phi$-ZER: Time Complexity Consideration}
 % \subsection{\texorpdfstring{$\phi$-ZER: Time Complexity Consideration}{phi-ZER: Time Complexity Consideration}}
 
% \noindent\textbf{Complexity Considerations for $k$-means in HE.} Figure~\ref{fig:all_by_num_data} illustrates the superiority of the kernel $k$-means algorithm over the general method in typical scenarios. Notably, at large values of $n$, kernel $k$-means, using the Boolean construction with the TFHE scheme, exhibits an $O(n^2)$ time complexity (refer to Table~\ref{tab:summary_complexity}). This complexity suggests a critical point in performance between the general and kernel methods. Consequently, the $\phi$-ZER framework should strategically choose the most efficient approach for $k$-means based on computed complexities. The $O(n^2)$ complexity arises from encrypted data point labels requiring multiple AND gate operations on the kernel matrix $\mathbf{K}$, in contrast to operations on the data matrix $\textbf{D}$ in the general method. Thus, a careful complexity assessment is vital for $k$-means, considering various factors like the number of clusters and ciphertext length.

\noindent\textbf{Special Cases with Critical Points.} 
While we have only presented results for ML algorithms that work best with the kernel approach in the HE domain, it is important to note that certain ML algorithms, such as LDA and linear regression, have critical decision boundaries that determine whether a general or kernel execution is preferred. These decision boundaries are determined by the matrix inverse operation, which dominates the time complexity over other operations such as matrix multiplication. Consequently, the kernel method may have lower performance than the general method due to the matrix inverse operation. However, this is a limitation that applies not only to the encrypted domain but also to the plain domain. Therefore, $\phi$-zer excludes LDA and linear regression from consideration since they cannot be efficiently executed using kernel-based approaches in either domain.

% \subsection{Future Work}
% Future optimizations for kernelized circuits can be explored at the hardware level to enhance the efficiency of ML training and STAT evaluations. Potential directions include:
% \begin{itemize}[leftmargin=0.35cm]
%    \item For BGV-like family schemes, \emph{rotation} of ciphertext is as critical as the multiplication operation since the rotation operation suffers a similar time complexity as the multiplication. Therefore, a suitable encoding method~\cite{cowan2021porcupine} could be considered to reduce the number of rotations in the kernelized circuit for high-end optimization.
%     \item Furthermore, the use of the \emph{lazy relinearization}~\cite{blatt2020optimized} technique could be explored. This technique performs only a small number of relinearizations after multiple multiplications to improve performance time.
%     \item Finally, the \emph{lineage tracing}~\cite{cui2000practical} can be applied to the kernel method. This optimization technique tracks the lineage of computations and reuses intermediate results to expedite the time performance.
% \end{itemize}

